Explaining Quantum Circuits with Shapley Values: Towards Explainable Quantum Machine Learning

Methods of artificial intelligence (AI) and especially machine learning (ML) have been growing ever more complex, and at the same time have more and more impact on people's lives. This leads to explainable AI (XAI) manifesting itself as an important research field that helps humans to better comprehend ML systems. In parallel, quantum machine learning (QML) is emerging with the ongoing improvement of quantum computing hardware combined with its increasing availability via cloud services. QML enables quantum-enhanced ML in which quantum mechanics is exploited to facilitate ML tasks, typically in the form of quantum-classical hybrid algorithms that combine quantum and classical resources. Quantum gates constitute the building blocks of gate-based quantum hardware and form circuits that can be used for quantum computations. For QML applications, quantum circuits are typically parameterized and their parameters are optimized classically such that a suitably defined objective function is minimized. Inspired by XAI, we raise the question of the explainability of such circuits by quantifying the importance of (groups of) gates for specific goals. To this end, we apply the well-established concept of Shapley values. The resulting attributions can be interpreted as explanations for why a specific circuit works well for a given task, improving the understanding of how to construct parameterized (or variational) quantum circuits, and fostering their human interpretability in general. An experimental evaluation on simulators and two superconducting quantum hardware devices demonstrates the benefits of the proposed framework for classification, generative modeling, transpilation, and optimization. Furthermore, our results shed some light on the role of specific gates in popular QML approaches.

==> declarations.tex <==
\subsection*{Funding}
Parts of this research have been funded by the Ministry of Science and Health of the State of Rhineland-Palatinate as part of the project \emph{AnQuC}.
Parts of this research have been funded by the Federal Ministry of Education and Research of Germany and the state of North-Rhine Westphalia as part of the \emph{Lamarr-Institute for Machine Learning and Artificial Intelligence}.
Access to quantum computing hardware has been funded by \emph{Fraunhofer Quantum Now}.

\subsection*{Competing interests}
The authors declare that they have no conflict of interest.

\subsection*{Authors' contributions}
All authors contributed to the writing and overall research process. R.H., S.Ml., M.J. and N.P. were responsible for the conceptualization. R.H., T.G. and S.Mc. wrote the software. R.H. developed the methodology. R.H. and T.G. performed the investigations. R.H. prepared the figures. N.P. was responsible for project administration. All authors reviewed the manuscript.

\subsection*{Availability of data and materials}
All data is publicly available online via the respective references.


